Evaluation of Test-Time Adaptation Under Computational Time Constraints

This paper proposes a novel online evaluation protocol for Test Time Adaptation (TTA) methods, which penalizes slower methods by providing them with fewer samples for adaptation. TTA methods leverage unlabeled data at test time to adapt to distribution shifts. Although many effective methods have been proposed, their impressive performance usually comes at the cost of significantly increased computation budgets. Current evaluation protocols overlook the effect of this extra computation cost, affecting their real-world applicability. To address this issue, we propose a more realistic evaluation protocol for TTA methods, where data is received in an online fashion from a constant-speed data stream, thereby accounting for the method's adaptation speed. We apply our proposed protocol to benchmark several TTA methods on multiple datasets and scenarios. Extensive experiments show that, when accounting for inference speed, simple and fast approaches can outperform more sophisticated but slower methods. For example, SHOT from 2020, outperforms the state-of-the-art method SAR from 2023 in this setting. Our results reveal the importance of developing practical TTA methods that are both accurate and efficient.

==> Figures/Lifelong/lifelong_graphs.tex <==

\begin{table*}[cc]

% \includegraphics[width=.3\linewidth]{Figures/Lifelong/ETA.pdf}&
% \includegraphics[width=.3\linewidth]{Figures/Lifelong/PL.pdf}&
% \includegraphics[width=.3\linewidth]{Figures/Lifelong/SAR.pdf}\\

% \includegraphics[width=.3\linewidth]{Figures/Lifelong/EATA.pdf}&
% \includegraphics[width=.3\linewidth]{Figures/Lifelong/TTAC-NQ.pdf} & \includegraphics[width=.3\linewidth]{Figures/Lifelong/COTTA.pdf} \\ 

% \includegraphics[width=.3\linewidth]{Figures/Lifelong/Tent.pdf}& \includegraphics[width=.3\linewidth]{Figures/Lifelong/SHOT.pdf}&
% \includegraphics[width=.3\linewidth]{Figures/Lifelong/SHOT-IM.pdf} \\ 
%  \includegraphics[width=.24\linewidth]{Figures/Lifelong/LifeLong_shot-order-0.pdf}&
% \includegraphics[width=.24\linewidth]{Figures/Lifelong/LifeLong_tent-order-0.pdf}&
% \includegraphics[width=.24\linewidth]{Figures/Lifelong/LifeLong_sar-order-0.pdf}&
% \includegraphics[width=.24\linewidth]{Figures/Lifelong/LifeLong_eata-order-0.pdf}&
% \includegraphics[width=.24\linewidth]{Figures/Lifelong/LifeLong_ttac_nq-order-0.pdf}\\

\includegraphics[width=0.5\linewidth]{Figures/Lifelong/LifeLong_LL-order-0-offline.pdf}&&
\includegraphics[width=0.5\linewidth]{Figures/Lifelong/LifeLong_LL-order-0-online.pdf}\\
\includegraphics[width=0.5\linewidth]{Figures/Lifelong/LifeLong_LL-order-1-offline.pdf}&&
\includegraphics[width=0.5\linewidth]{Figures/Lifelong/LifeLong_LL-order-1-online.pdf}\\
% \includegraphics[width=0.5\linewidth]{Figures/Lifelong/LifeLong_LL-order-2-offline.pdf}&&
% \includegraphics[width=0.5\linewidth]{Figures/Lifelong/LifeLong_LL-order-2-online.pdf}\\
\caption{\textbf{Continual setup evaluation:} left offline, right online each row is a different order}
\end{table*}

==> Figures/Table_to_Fig/tabel_fig.tex <==
\begin{figure}
    \centering
    \includegraphics[width=0.95\columnwidth,height=0.3\textwidth]{Figures/Table_to_Fig/table_fig.pdf}
    \caption{\textbf{Sample table info fig.} }
    \label{fig:pull_fig}
\end{figure}
% \begin{figure}
%     \centering
%     \includegraphics[width=0.95\columnwidth,height=0.3\textwidth]{Figures/Table_to_Fig/table_fig_eps.pdf}
%     \caption{\textbf{Sample table info fig.} }
%     \label{fig:pull_fig}
% \end{figure}

==> Figures/stream_speed/stream_speed_single.tex <==
\begin{figure}
    \centering
    \includegraphics[width=0.95\columnwidth]{Figures/stream_speed/Stream_speed_Single.pdf}
    \caption{\textbf{Stream Speed Variation for the Single Model Setup} }
    \label{fig:stream_speed_single}
\end{figure}

==> Sections/delete.tex <==
\section{Introduction}
In recent years, Deep Neural Networks (DNNs) have demonstrated remarkable success in various tasks~\cite{he2016deep} thanks to their ability to learn from large datasets~\cite{deng2009imagenet}. 

However, a significant limitation of DNNs is their low performance when tested on out-of-distribution data, which violates the i.i.d. assumption~\cite{imagenetr,imagenetc,3dcc} (the training and testing data are from the same distribution). 

Such failure cases are concerning, since distribution shifts are common in real-world applications, \eg image corruptions~\cite{imagenetc}, changing weather conditions~\cite{sakaridis2021acdc}, or security breaches~\cite{goodfellow2014explaining}. 

Test Time Adaptation (TTA) ~\cite{saenko2010adapting, ttt, liu2021ttt++} has demonstrated promising results for solving the above problem.
TTA leverages the unlabeled data that arrives at test time by adapting the forward pass of pre-trained DNNs according to some proxy task~\cite{shot,pl}.
Though recent methods have made significant progress at improving accuracy under distribution shifts~\cite{tent,eata,dda}, many of them incur high computational overhead. 
For instance, some methods require self-supervised fine-tuning on the data~\cite{chen2022contrastive}, while others perform a diffusion process per input~\cite{dda}. 
The computational overhead of TTA methods can decrease their inference speed, which is a critical property in many real-world applications. 
This property, however, is overlooked in the current evaluation protocols for TTA methods. % overlooks this practical issue by evaluating them in an offline fashion.
In particular, they assume an \textit{offline} setting, which neglects how % the practical impact that decreased inference speed has in real-world scenarios. %  where domain shifts occur.
 events constantly unfold regardless of the model's speed, causing the model to miss incoming samples when it is busy processing previous ones.
For TTA methods that adapt using test data, % for adaptation, 
missing samples has a direct effect on the method's accuracy, as it will have fewer samples for adaptation. 
That is, the slower the TTA method, the fewer samples it can leverage for adapting to the distribution shift.
Thus, the current offline protocol for evaluating TTA methods 
is unsuitable for assessing the effectiveness and applicability of these methods in the real world. 
In this work, we propose a novel \textit{online} evaluation protocol that factors in inference speed to assess the real-world applicability of TTA methods. 
Our evaluation protocol is inspired by Online Learning settings~\cite{cloc, shalev2012online} and mimics real-world scenarios by exposing all TTA methods to a constant-speed stream of data. 
Under this setup, the performance of slow TTA methods is intrinsically penalized, as the time spent adapting on a sample implies the method misses other samples that could have been useful for adaptation.
Specifically, our protocol dictates that if a method $g_{\text{slow}}$ is $k$ times slower than the stream, then 
it may only use every $k^{\text{th}}$ sample for adaptation. 
In contrast, a method $g_{\text{fast}}$ that is as fast as the stream is allowed to adapt to every sample. 
Figure \ref{fig:pull_fig} shows the effect of evaluating several methods under our online protocol, where slower methods are penalized and faster but simpler methods become better alternatives.

We apply our proposed evaluation protocol to benchmark several TTA methods on multiple datasets, and provide a fair assessment of their performance subject to the realistic consequences of slowing inference speeds. 
Our experimental results highlight the importance of developing TTA methods that adapt to distribution shifts with minimal impacts on inference speed. 
Our contributions are twofold:\\

\vspace{-6pt}\textbf{(i)} We propose an online evaluation protocol for TTA methods that penalizes slow methods by providing them with fewer samples for adaptation. 
Our approach is simple yet effective for assessing the effectiveness of TTA methods in scenarios where data come as a constant-speed stream.\\

\vspace{-6pt}\textbf{(ii)} Following our proposed protocol, we provide a comprehensive experimental analysis of 15 TTA methods evaluated on 3 large-scale datasets and under 3 different evaluation scenarios.
These scenarios consider adaptation to a single domain and continual adaptation to several domains. 
Our analysis shows that, when inference speed is accounted for, simple (but fast) approaches can benefit from adapting on more data, and thus outperform more sophisticated (but slow) methods.
We hope our evaluation scheme inspires ensuing TTA methods to consider inference speed as a critical dimension that directly affects the real-world performance of methods.

Upon acceptance of the paper, we will release the PyTorch~\cite{NEURIPS2019_9015} implementation of our online evaluation protocol to foster realistic evaluations of TTA methods.


==> Tables/episodic_evaluation_old.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
% \begin{table*}[]
% \caption{\label{tab:imagenetc} \textbf{Evaluation on ImageNetc.}
% We...}
% \resizebox{\textwidth}{!}{
% \setlength{\tabcolsep}{5.0pt}
% \begin{tabular}{cc|ccc|cccc|cccc|cccc|g}
% \toprule
% \multirow{2}{*}{Method} & \multirow{2}{*}{Eval.} & \multicolumn{3}{c|}{Noise} & \multicolumn{4}{c|}{Blur}        & \multicolumn{4}{c|}{Weather}  & \multicolumn{4}{c|}{Digital}          &                         \\ 
%                         &                        & gauss.  & shot  & impul.  & defoc. & glass & mot. & zoom & snow & frost & fog & bright. & contr. & elast. & pixel. & jpeg & \multirow{-2}{*}{Avg.} \\ \midrule
% % & & \multicolumn{3}{|ccc|}{Noise} &\multicolumn{4}{|cccc|}{Blur} & \multicolumn{4}{|cccc|}{Weather} & \multicolumn{4}{|cccc|}{Digital} & \\
% % Method                   & Eval. & gauss.               & shot                 & impul.              & defocus              & glass                & motion               & zoom                 & snow                 & frost                & fog                   & bright.            & contrast             & elastic              & pixelate             & jpeg                 & Avg.              \\ \midrule
% Source                    & Online                    & 97.8                 & 97.1                 & 98.1                 & 82.1                 & 90.2                 & 85.2                 & 77.5                 & 83.1                 & 76.7                 & 75.6                  & 41.1                  & 94.6                 & 83.0                 & 79.4                 & 68.4                 & 82.0                 \\
% \midrule AdaBN                    & Online                    & 84.9                 & 84.3                 & 84.3                 & 85.0                 & 84.7                 & 73.6                 & 61.1                 & 65.8                 & 66.9                 & 52.1                  & 34.8                  & 83.3                 & 56.1                 & 51.1                 & 60.3                 & 68.5                 \\
% \midrule LAME                     & Online                    & 98.31 & 97.55 & 98.59 & 82.39 & 90.91 & 86.06 & 78.08 & 84.46 & 77.49 & 77.32 & 41.38 & 94.79 & 84.76 & 80.04 & 68.91  & 82.74                 \\
% \midrule BN             & Online                    & 84.6                 & 83.9                 & 83.8                 & 80.1                 & 80.2                 & 71.7                 & 60.4                 & 65.4                 & 65.2                 & 51.6                  & 34.6                  & 76.3                 & 54.4                 & 49.7                 & 59.2                 & 66.7                 \\
% \midrule \multirow{2}{*}{Tent}    & Offline                  & 71.3                 & 69.4                 & 70.2                 & 72.0                 & 72.9                 & 58.7                 & 50.7                 & 52.8                 & 58.8                 & 42.7                  & 32.7                  & 73.3                 & 45.5                 & 41.5                 & 47.7                 & 57.3                 \\
%                          & Online                    & 75.7                 & 78.3                 & 75.2                 & 76.3                 & 77.3                 & 64.6                 & 55.6                 & 57.3                 & 61.4                 & 45.9                  & 33.5                  & 77.1                 & 50.1                 & 44.2                 & 51.4                 & 61.6                 \\
% \midrule \multirow{2}{*}{ETA}     & Offline                  & 64.9                 & 62.7                 & 63.6                 & 66.4                 & 66.3                 & 52.4                 & 47.3                 & 48.2                 & 54.1                 & 40.2                  & 32.2                  & 54.8                 & 42.3                 & 39.2                 & 44.7                 &\textbf{ 52.0 }                \\
%                          & Online                    & 70.2	&67.3	&69.1	&72.2	&72.1	&56.6	&50.0	&52.6	&56.9	&42.0	&32.5	&61.7	&45.0	&41.3	&47.4	&55.8                 \\
% \midrule \multirow{2}{*}{EATA}    & Offline                  & 65.5                 & 62.4                 & 63.5                 & 66.6                 & 67.2                 & 52.0                 & 47.3                 & 48.2                 & 54.1                 & 39.9                  & 32.1                  & 55.0                 & 42.3                 & 39.2                 & 44.8                 & \textbf{52.0}                 \\
%                          & Online                    &69.3	&67.1&	69.2&	71.1&	71.7&	57.5&	49.9&	51.9&	57.4&	42.4&	32.6&	60.7&	45.1&	41.4&	47.4&	55.6                 \\
% \midrule \multirow{2}{*}{TTAC-NQ} & Offline                  & 71.3                 & 70.3                 & 70.8                 & 82.1                 & 77.4                 & 63.9                 & 53.9                 & 49.9                 & 55.5                 & 43.9                  & 32.8                  & 81.4                 & 43.7                 & 41.1                 & 46.7                 & 59.0                 \\
%                          & Online                    & 79.4                 & 75.7                 & 78.9                 & 86.6                 & 86.2                 & 77.1                 & 61.8                 & 58.8                 & 62.4                 & 51.5                  & 34.4                  & 88.5                 & 52.1                 & 49.1                 & 55.5                 & 66.5                 \\
% \midrule \multirow{2}{*}{MEMO}    & Offline                  & 92.5                 & 91.3                 & 91.0                 & 84.0                 & 87.0                 & 79.3                 & 72.4                 & 74.6                 & 71.3                 & 67.9                  & 39.0                  & 89.0                 & 76.2                 & 67.0                 & 62.4                 & 76.3                 \\
%                          & Online                    & 97.7                 & 97.0                 & 98.0                 & 82.1                 & 90.1                 & 85.1                 & 77.4                 & 83.0                 & 76.6                 & 75.4                  & 41.0                  & 94.5                 & 82.9                 & 79.2                 & 68.2                 & 81.9                 \\
% \midrule \multirow{2}{*}{COTTA}   & Offline                  & 78.4                 & 77.8                 & 77.2                 & 80.5                 & 79.1                 & 64.0                 & 53.3                 & 57.8                 & 60.7                 & 44.1                  & 32.9                  & 73.1                 & 48.6                 & 42.3                 & 52.6                 & 61.5                 \\
%                          & Online                    & 82.9                 & 81.6                 & 81.9                 & 87.4                 & 85.6                 & 75.6                 & 61.1                 & 63.1                 & 64.9                 & 49.9                  & 34.8                  & 91.2                 & 54.0                 & 48.8                 & 56.6                 & 68.0                 \\
% \midrule \multirow{2}{*}{SHOT}    & Offline                  & 73.4                 & 70.2                 & 73.0                 & 76.6                 & 75.5                 & 59.8                 & 53.8                 & 54.2                 & 63.4                 & 44.7                  & 35.5                  & 79.3                 & 46.9                 & 43.2                 & 49.7                 & 59.9                 \\
%                          & Online                    & 73.6                 & 69.0                 & 71.1                 & 74.6                 & 74.8                 & 60.0                 & 52.9                 & 54.1                 & 61.3                 & 44.1                  & 34.1                  & 77.8                 & 46.8                 & 43.1                 & 49.2                 & \textbf{59.1}                 \\
% \midrule \multirow{2}{*}{SAR}     & Offline                  & 69.5                 & 69.7                 & 69.0                 & 71.2                 & 71.7                 & 58.1                 & 50.5                 & 52.9                 & 57.9                 & 42.7                  & 32.7                  & 62.9                 & 45.5                 & 41.6                 & 47.8                 & 56.2                 \\
%                          & Online                    & 84.8                 & 84.2                 & 84.0                 & 84.9                 & 84.4                 & 73.4                 & 60.8                 & 65.6                 & 66.7                 & 51.9                  & 34.8                  & 83.1                 & 56.0                 & 50.9                 & 60.1                 & 68.4                 \\ 
% \midrule \multirow{2}{*}{DDA}     & Offline            &      58.6    & 57.8  & 59.0    & 87.0    & 81.6  & 76.6   & 65.9 & 67.9 & 66.7  & 64.0 & 40.0    & 92.2     & 52.2    & 46.6     & 49.9 & 64.4  \\ 
%                          & Online &97.8	& 97.0 &	98.1&	82.1	& 90.2 &	85.2&	77.5	& 83.1 &	76.7&	75.6	& 41.1 &	94.6&	83.0	&79.4 & 68.3&	82.0    \\                
%                          % & 85.1    & 84.6  & 84.5    & 85.3    & 85.1  & 74.4   & 61.9 & 66.2 & 67.5  & 52.7 & 35.3    & 83.6     & 56.7    & 51.6     & 60.7 & 69.0  \\ 
%                          % \cmidrule(l){2-18}
%                          % \midrule
%                          \bottomrule
% \end{tabular}
% }
% \end{table*}

\begin{table*}[]
\caption{\label{tab:imagenetc_episodic} \textbf{Episodic Evaluation on ImageNet-C.}
We...}
\resizebox{\textwidth}{!}{
\setlength{\tabcolsep}{5.0pt}
\begin{tabular}{cc|ccc|cccc|cccc|cccc|g}
\toprule
\multirow{2}{*}{Method} & \multirow{2}{*}{Eval.} & \multicolumn{3}{c|}{Noise} & \multicolumn{4}{c|}{Blur}        & \multicolumn{4}{c|}{Weather}  & \multicolumn{4}{c|}{Digital}          &                         \\ 
                        &                        & gauss.  & shot  & impul.  & defoc. & glass & motion & zoom & snow & frost & fog & brigh. & contr. & elast. & pixel. & jpeg & \multirow{-2}{*}{Avg.} \\ \midrule
% & & \multicolumn{3}{|ccc|}{Noise} &\multicolumn{4}{|cccc|}{Blur} & \multicolumn{4}{|cccc|}{Weather} & \multicolumn{4}{|cccc|}{Digital} & \\
% Method                   & Eval. & gauss.               & shot                 & impul.              & defocus              & glass                & motion               & zoom                 & snow                 & frost                & fog                   & bright.            & contrast             & elastic              & pixelate             & jpeg                 & Avg.              \\ \midrule
Source                    & Online                    & 97.8                 & 97.1                 & 98.1                 & 82.1                 & 90.2                 & 85.2                 & 77.5                 & 83.1                 & 76.7                 & 75.6                  & 41.1                  & 94.6                 & 83.0                 & 79.4                 & 68.4                 & 82.0                 \\
\midrule AdaBN                    & Online                    & 84.9                 & 84.3                 & 84.3                 & 85.0                 & 84.7                 & 73.6                 & 61.1                 & 65.8                 & 66.9                 & 52.1                  & 34.8                  & 83.3                 & 56.1                 & 51.1                 & 60.3                 & 68.5                 \\
\midrule LAME                     & Online                    & 85.0                 & 84.3                 & 84.3                 & 85.0                 & 84.7                 & 73.7                 & 61.2                 & 65.8                 & 67.0                 & 52.1                  & 34.8                  & 83.4                 & 56.3                 & 51.2                 & 60.3                 & 68.6                 \\
\midrule BN             & Online                    & 84.6                 & 83.9                 & 83.8                 & 80.1                 & 80.2                 & 71.7                 & 60.4                 & 65.4                 & 65.2                 & 51.6                  & 34.6                  & 76.3                 & 54.4                 & 49.7                 & 59.2                 & 66.7                 \\
\midrule
\midrule \multirow{2}{*}{SHOT}    & Offline                  & 73.4                 & 70.2                 & 73.0                 & 76.6                 & 75.5                 & 59.8                 & 53.8                 & 54.2                 & 63.4                 & 44.7                  & 35.5                  & 79.3                 & 46.9                 & 43.2                 & 49.7                 & 59.9                 \\
                         & Online                    & 73.6                 & 69.0                 & 71.1                 & 74.6                 & 74.8                 & 60.0                 & 52.9                 & 54.1                 & 61.3                 & 44.1                  & 34.1                  & 77.8                 & 46.8                 & 43.1                 & 49.2                 & \textbf{59.1}                 \\
\midrule \multirow{2}{*}{Tent}    & Offline                  & 71.3                 & 69.4                 & 70.2                 & 72.0                 & 72.9                 & 58.7                 & 50.7                 & 52.8                 & 58.8                 & 42.7                  & 32.7                  & 73.3                 & 45.5                 & 41.5                 & 47.7                 & 57.3                 \\
                         & Online                    & 75.7                 & 78.3                 & 75.2                 & 76.3                 & 77.3                 & 64.6                 & 55.6                 & 57.3                 & 61.4                 & 45.9                  & 33.5                  & 77.1                 & 50.1                 & 44.2                 & 51.4                 & 61.6                 \\
% \midrule \multirow{2}{*}{ETA}     & Offline                  & 64.9                 & 62.7                 & 63.6                 & 66.4                 & 66.3                 & 52.4                 & 47.3                 & 48.2                 & 54.1                 & 40.2                  & 32.2                  & 54.8                 & 42.3                 & 39.2                 & 44.7                 &\textbf{ 52.0 }                \\
%                          & Online                    & 70.2	&67.3	&69.1	&72.2	&72.1	&56.6	&50.0	&52.6	&56.9	&42.0	&32.5	&61.7	&45.0	&41.3	&47.4	&55.8                 \\
\midrule \multirow{2}{*}{SAR}     & Offline                  & 69.5                 & 69.7                 & 69.0                 & 71.2                 & 71.7                 & 58.1                 & 50.5                 & 52.9                 & 57.9                 & 42.7                  & 32.7                  & 62.9                 & 45.5                 & 41.6                 & 47.8                 & 56.2                 \\
                         & Online                    & 84.8                 & 84.2                 & 84.0                 & 84.9                 & 84.4                 & 73.4                 & 60.8                 & 65.6                 & 66.7                 & 51.9                  & 34.8                  & 83.1                 & 56.0                 & 50.9                 & 60.1                 & 68.4                 \\ 
\midrule \multirow{2}{*}{COTTA}   & Offline                  & 78.4                 & 77.8                 & 77.2                 & 80.5                 & 79.1                 & 64.0                 & 53.3                 & 57.8                 & 60.7                 & 44.1                  & 32.9                  & 73.1                 & 48.6                 & 42.3                 & 52.6                 & 61.5                 \\
                         & Online                    & 82.9                 & 81.6                 & 81.9                 & 87.4                 & 85.6                 & 75.6                 & 61.1                 & 63.1                 & 64.9                 & 49.9                  & 34.8                  & 91.2                 & 54.0                 & 48.8                 & 56.6                 & 68.0                 \\
\midrule
\midrule \multirow{2}{*}{TTAC-NQ} & Offline                  & 71.3                 & 70.3                 & 70.8                 & 82.1                 & 77.4                 & 63.9                 & 53.9                 & 49.9                 & 55.5                 & 43.9                  & 32.8                  & 81.4                 & 43.7                 & 41.1                 & 46.7                 & 59.0                 \\
                         & Online                    & 79.4                 & 75.7                 & 78.9                 & 86.6                 & 86.2                 & 77.1                 & 61.8                 & 58.8                 & 62.4                 & 51.5                  & 34.4                  & 88.5                 & 52.1                 & 49.1                 & 55.5                 & 66.5                 \\
\midrule \multirow{2}{*}{EATA}    & Offline                  & 65.5                 & 62.4                 & 63.5                 & 66.6                 & 67.2                 & 52.0                 & 47.3                 & 48.2                 & 54.1                 & 39.9                  & 32.1                  & 55.0                 & 42.3                 & 39.2                 & 44.8                 & \textbf{52.0}                 \\
                         & Online                    &69.3	&67.1&	69.2&	71.1&	71.7&	57.5&	49.9&	51.9&	57.4&	42.4&	32.6&	60.7&	45.1&	41.4&	47.4&	55.6                 \\
                         \midrule
\midrule \multirow{2}{*}{MEMO}    & Offline                  & 92.5                 & 91.3                 & 91.0                 & 84.0                 & 87.0                 & 79.3                 & 72.4                 & 74.6                 & 71.3                 & 67.9                  & 39.0                  & 89.0                 & 76.2                 & 67.0                 & 62.4                 & 76.3                 \\
                         & Online                    & 97.7                 & 97.0                 & 98.0                 & 82.1                 & 90.1                 & 85.1                 & 77.4                 & 83.0                 & 76.6                 & 75.4                  & 41.0                  & 94.5                 & 82.9                 & 79.2                 & 68.2                 & 81.9                 \\
\midrule \multirow{2}{*}{DDA}     & Offline            &      58.6    & 57.8  & 59.0    & 87.0    & 81.6  & 76.6   & 65.9 & 67.9 & 66.7  & 64.0 & 40.0    & 92.2     & 52.2    & 46.6     & 49.9 & 64.4  \\ 
                         & Online &97.8	& 97.0 &	98.1&	82.1	& 90.2 &	85.2&	77.5	& 83.1 &	76.7&	75.6	& 41.1 &	94.6&	83.0	&79.4 & 68.3&	82.0    \\                
                         % & 85.1    & 84.6  & 84.5    & 85.3    & 85.1  & 74.4   & 61.9 & 66.2 & 67.5  & 52.7 & 35.3    & 83.6     & 56.7    & 51.6     & 60.7 & 69.0  \\ 
                         % \cmidrule(l){2-18}
                         % \midrule
                         \midrule\bottomrule
\end{tabular}
}
\end{table*}

==> Tables/episodic_evaluation_v2.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table.xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option. i.e. \documentclass[xcolor=table]{beamer}
\begin{table*}[]
\caption{\label{tab:imagenetc_episodic} \textbf{Episodic Evaluation on ImageNet-C.}
We...}
\resizebox{\textwidth}{!}{
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table.xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option. i.e. \documentclass[xcolor=table]{beamer}

\begin{tabular}{c|c|ccc|cccc|cccc|cccc|c}
\toprule
\rowcolor[HTML]{FFFFFF} 
\cellcolor[HTML]{FFFFFF}                          & \cellcolor[HTML]{FFFFFF}                        & \multicolumn{3}{c|}{\cellcolor[HTML]{FFFFFF}Noise} & \multicolumn{4}{c|}{\cellcolor[HTML]{FFFFFF}Blur}                           & \multicolumn{4}{c|}{\cellcolor[HTML]{FFFFFF}Weather} & \multicolumn{4}{c|}{\cellcolor[HTML]{FFFFFF}Digital} & \cellcolor[HTML]{FFFFFF}                       \\
\rowcolor[HTML]{FFFFFF} 
\multirow{-2}{*}{\cellcolor[HTML]{FFFFFF}Method}  & \multirow{-2}{*}{\cellcolor[HTML]{FFFFFF}Online} & gauss.                         & shot   & impul.  & defoc.                       & glass & motion                       & zoom & snow       & frost       & fog        & brigh.      & contr.      & elast.      & pixel.      & jpeg      & \multirow{-2}{*}{\cellcolor[HTML]{FFFFFF}Avg.} \\
\midrule
\rowcolor[HTML]{FFFFFF} 
Source                                            & \cmark                                          & 97.8                           & 97.1   & 98.1    & 82.1                         & 90.2  & 85.2                         & 77.5 & 83.1       & 76.7        & 75.6       & 41.1        & 94.6        & 83.0        & 79.4        & 68.4      & 82.0                                           \\
\rowcolor[HTML]{FFFFFF} 
AdaBN                                             & \cmark                                          & 84.9                           & 84.3   & 84.3    & 85.0                         & 84.7  & 73.6                         & 61.1 & 65.8       & 66.9        & 52.1       & 34.8        & 83.3        & 56.1        & 51.1        & 60.3      & 68.5                                           \\
\rowcolor[HTML]{FFFFFF} 
LAME                                              & \cmark                                         & 98.3 & 97.6 & 98.6 & 82.4 & 90.9 & 86.1 & 78.1 & 84.5 & 77.5 & 77.3 & 41.4 & 94.8 & 84.8 & 80.0 & 68.9  & 82.7                                           \\
\rowcolor[HTML]{FFFFFF} 
BN                                                & \cmark                                          & 84.6                           & 83.9   & 83.8    & 80.1                         & 80.2  & 71 .7                         & 60.4 & 65.4       & 65.2        & 51.6       & 34.6        & 76.3        & 54.4        & 49.7        & 59.2      & 66.7                                           \\
\midrule
\midrule
\rowcolor[HTML]{fdf2f3} 
\cellcolor[HTML]{FFFFFF}                          & \cellcolor[HTML]{FFFFFF}\xmark                 & \cellcolor[HTML]{e9f5f9}73.4   & 70.2   & 73.0    & 76.6                         & 75.5  & \cellcolor[HTML]{e9f5f9}59.8 & 53.8 & 54.2       & 63.4        & 44.7       & 35.5        & 79.3        & 46.9        & 43.2        & 49.7      & 59.9                                           \\
\rowcolor[HTML]{e9f5f9} 
\multirow{-2}{*}{\cellcolor[HTML]{FFFFFF}SHOT}    & \cellcolor[HTML]{FFFFFF}\cmark                  & \cellcolor[HTML]{fdf2f3}73.6   & 69.0   & 71.1    & 74.6                         & 74.8  & \cellcolor[HTML]{fdf2f3}60.0 & 52.9 & 54.1       & 61.3        & 44.1       & 34.1        & 77.8        & 46.8        & 43.1        & 49.2      & 59.1                                           \\
\midrule
\rowcolor[HTML]{e9f5f9} 
\cellcolor[HTML]{FFFFFF}                          & \cellcolor[HTML]{FFFFFF}\xmark                 & 71.3                           & 69.4   & 70.2    & 72.0                         & 72.9  & 58.7                         & 50.7 & 52.8       & 58.8        & 42.7       & 32.7        & 73.3        & 45.5        & 41.5        & 47.7      & 57.3                                           \\
\rowcolor[HTML]{fdf2f3} 
\multirow{-2}{*}{\cellcolor[HTML]{FFFFFF}Tent}    & \cellcolor[HTML]{FFFFFF}\cmark                  & 75.7                           & 78.3   & 75.2    & 76.3                         & 77.3  & 64.6                         & 55.6 & 57.3       & 61.4        & 45.9       & 33.5        & 77.1        & 50.1        & 44.2        & 51.4      & 61.6                                           \\
\midrule
\rowcolor[HTML]{e9f5f9} 
\cellcolor[HTML]{FFFFFF}                          & \cellcolor[HTML]{FFFFFF}\xmark                 & 69.5                           & 69.7   & 69.0    & 71.2                         & 71.7  & 58.1                         & 50.5 & 52.9       & 57.9        & 42.7       & 32.7        & 62.9        & 45.5        & 41.6        & 47.8      & 56.2                                           \\
\rowcolor[HTML]{fdf2f3} 
\multirow{-2}{*}{\cellcolor[HTML]{FFFFFF}SAR}     & \cellcolor[HTML]{FFFFFF}\cmark                  & 84.8                           & 84.2   & 84.0    & 84.9                         & 84.4  & 73.4                         & 60.8 & 65.6       & 66.7        & 51.9       & 34.8        & 83.1        & 56.0        & 50.9        & 60.1      & 68.4                                           \\
\midrule
\rowcolor[HTML]{e9f5f9} 
\cellcolor[HTML]{FFFFFF}                          & \cellcolor[HTML]{FFFFFF}\xmark                 & 78.4                           & 77.8   & 77.2    & 80.5                         & 79.1  & 64.0                         & 53.3 & 57.8       & 60.7        & 44.1       & 32.9        & 73.1        & 48.6        & 42.3        & 52.6      & 61.5                                           \\
\rowcolor[HTML]{fdf2f3} 
\multirow{-2}{*}{\cellcolor[HTML]{FFFFFF}COTTA}   & \cellcolor[HTML]{FFFFFF}\cmark                  & 82.9                           & 81.6   & 81.9    & 87.4                         & 85.6  & 75.6                         & 61.1 & 63.1       & 64.9        & 49.9       & 34.8        & 91.2        & 54.0        & 48.8        & 56.6      & 68.0                                           \\
\midrule\midrule
\rowcolor[HTML]{e9f5f9} 
\cellcolor[HTML]{FFFFFF}                          & \cellcolor[HTML]{FFFFFF}\xmark                 & 71.3                           & 70.3   & 70.8    & 82.1                         & 77.4  & 63.9                         & 53.9 & 49.9       & 55.5        & 43.9       & 32.8        & 81.4        & 43.7        & 41.1        & 46.7      & 59.0                                           \\
\rowcolor[HTML]{fdf2f3} 
\multirow{-2}{*}{\cellcolor[HTML]{FFFFFF}TTAC-NQ} & \cellcolor[HTML]{FFFFFF}\cmark                  & 79.4                           & 75.7   & 78.9    & 86.6                         & 86.2  & 77.1                         & 61.8 & 58.8       & 62.4        & 51.5       & 34.4        & 88.5        & 52.1        & 49.1        & 55.5      & 66.5                                           \\
\midrule
\rowcolor[HTML]{e9f5f9} 
\cellcolor[HTML]{FFFFFF}                          & \cellcolor[HTML]{FFFFFF}\xmark                 & 65.5                           & 62.4   & 63.5    & 66.6                         & 67.2  & 52.0                         & 47.3 & 48.2       & 54.1        & 39.9       & 32.1        & 55.0        & 42.3        & 39.2        & 44.8      & 52.0                                           \\
\rowcolor[HTML]{fdf2f3} 
\multirow{-2}{*}{\cellcolor[HTML]{FFFFFF}EATA}    & \cellcolor[HTML]{FFFFFF}\cmark                  & 69.3                           & 67.1   & 69.2    & 71.1                         & 71.7  & 57.5                         & 49.9 & 51.9       & 57.4        & 42.4       & 32.6        & 60.7        & 45.1        & 41.4        & 47.4      & 55.6                                           \\
\midrule
\rowcolor[HTML]{e9f5f9} 
\cellcolor[HTML]{FFFFFF}                          & \cellcolor[HTML]{FFFFFF}\xmark                 & 92.5                           & 91.3   & 91.0    & \cellcolor[HTML]{fdf2f3}84.0 & 87.0  & 79.3                         & 72.4 & 74.6       & 71.3        & 67.9       & 39.0        & 89.0        & 76.2        & 67.0        & 62.4      & 76.3                                           \\
\rowcolor[HTML]{fdf2f3} 
\multirow{-2}{*}{\cellcolor[HTML]{FFFFFF}MEMO}    & \cellcolor[HTML]{FFFFFF}\cmark                  & 97.7                           & 97.0   & 98.0    & \cellcolor[HTML]{e9f5f9}82.1 & 90.1  & 85.1                         & 77.4 & 83.0       & 76.6        & 75.4       & 41.0        & 94.5        & 82.9        & 79.2        & 68.2      & 81.9                                           \\
\midrule
\rowcolor[HTML]{e9f5f9} 
\cellcolor[HTML]{FFFFFF}                          & \cellcolor[HTML]{FFFFFF}\xmark                 & 58.6                           & 57.8   & 59.0    & \cellcolor[HTML]{fdf2f3}87.0 & 81.6  & 76.6                         & 65.9 & 67.9       & 66.7        & 64.0       & 40.0        & 92.2        & 52.2        & 46.6        & 49.9      & 64.4                                           \\
\rowcolor[HTML]{fdf2f3} 
\multirow{-2}{*}{\cellcolor[HTML]{FFFFFF}DDA}     & \cellcolor[HTML]{FFFFFF}\cmark                  & 97.8                           & 97.0   & 98.1    & \cellcolor[HTML]{e9f5f9}82.1 & 90.2  & 85.2                         & 77.5 & 83.1       & 76.7        & 75.6       & 41.1        & 94.6        & 83.0        & 79.4        & 68.3      & 82.0                                          \\ \midrule \bottomrule
\end{tabular}
}
\end{table*}

==> Tables/lifelong_evaluation.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
% \usepackage{graphicx}
\begin{table*}[]
\resizebox{\textwidth}{!}{%
\begin{tabular}{cl|ccccccccccccccc|c|g}
\toprule
\multicolumn{2}{c}{}&\multicolumn{15}{c}{$\xrightarrow{\makebox[20cm]{t}}$}
\\
\multirow{2}{*}{Method}        & \multicolumn{1}{c|}{\multirow{2}{*}{Eval.}} & \multicolumn{3}{c|}{Noise}                                                 & \multicolumn{4}{c|}{Blur}                                                                        & \multicolumn{4}{c|}{Weather}                                                                         & \multicolumn{4}{c|}{Digital}                                                               & \multirow{2}{*}{val}  & \multirow{2}{*}{Avg.} \\
                               & \multicolumn{1}{c|}{}                       & gaussian             & shot                 & \multicolumn{1}{c|}{impulse} & defocus              & glass                & motion               & \multicolumn{1}{c|}{zoom}   & snow                 & frost                & fog                  & \multicolumn{1}{c|}{brightness} & contrast             & elastic              & pixelate             & jpeg                  &                       &                          \\ \midrule
\multirow{2}{*}{Tent}          & reproduce                                   & 71.308               & 65.862               & \multicolumn{1}{c|}{68.694}  & 81.912               & 89.198               & 93.912               & \multicolumn{1}{c|}{96.336} & 98.758               & 99.306               & 99.286               & \multicolumn{1}{c|}{99.232}     & 99.608               & 99.462               & 99.438               & 99.472                & 99.346                & 91.320625                \\ %\cmidrule(l){3-19} 
                               & online                                      & 72.342               & 65.77                & \multicolumn{1}{c|}{68.54}   & 81.522               & 88.832               & 93.732               & \multicolumn{1}{c|}{96.326} & 98.798               & 99.332               & 99.308               & \multicolumn{1}{c|}{99.194}     & 99.606               & 99.444               & 99.424               & 99.466                & 99.36                 & 91.31225                 \\ \midrule
\multirow{2}{*}{AdaBN}         & reproduce                                   & 84.914               & 84.05                & \multicolumn{1}{c|}{84.27}   & 84.882               & 84.738               & 73.662               & \multicolumn{1}{c|}{61.246} & 65.71                & 66.972               & 52.032               & \multicolumn{1}{c|}{34.784}     & 82.998               & 56.01                & 51.03                & 60.152                & 24.77                 & 65.76375                 \\ %\cmidrule(l){3-19} 
                               & online                                      & 84.914               & 84.05                & \multicolumn{1}{c|}{84.27}   & 84.882               & 84.738               & 73.662               & \multicolumn{1}{c|}{61.246} & 65.71                & 66.972               & 52.032               & \multicolumn{1}{c|}{34.784}     & 82.998               & 56.01                & 51.03                & 60.152                & 24.77                 & 65.76375                 \\ \midrule
\multirow{2}{*}{ETA}           & reproduce                                   & 65.216               & 59.262               & \multicolumn{1}{c|}{60.504}  & 70.086               & 68.332               & 62.976               & \multicolumn{1}{c|}{56.336} & 58.852               & 61.066               & 48.4                 & \multicolumn{1}{c|}{39.248}     & 58.132               & 48.904               & 44.884               & 48.644                & 32.896                & 55.233625                \\ %\cmidrule(l){3-19} 
                               & online                                      & 77.114               & 67.52                & \multicolumn{1}{c|}{65.942}  & 75.386               & 70.678               & 64.758               & \multicolumn{1}{c|}{57.634} & 63.2                 & 62.556               & 52.904               & \multicolumn{1}{c|}{40.156}     & 64.18                & 50.602               & 46.576               & 50.116                & 32.482                & 58.86275                 \\ \midrule
\multirow{2}{*}{EATA}          & reproduce                                   & 65.216               & 59.262               & \multicolumn{1}{c|}{60.504}  & 70.086               & 68.332               & 62.976               & \multicolumn{1}{c|}{56.336} & 58.852               & 61.066               & 48.4                 & \multicolumn{1}{c|}{39.248}     & 58.132               & 48.904               & 44.884               & 48.644                & 32.896                & 55.233625                \\ %\cmidrule(l){3-19} 
                               & online                                      & 77.114               & 67.52                & \multicolumn{1}{c|}{65.942}  & 75.386               & 70.678               & 64.758               & \multicolumn{1}{c|}{57.634} & 63.2                 & 62.556               & 52.904               & \multicolumn{1}{c|}{40.156}     & 64.18                & 50.602               & 46.576               & 50.116                & 32.482                & 58.86275                 \\ \midrule
\multirow{2}{*}{TTAC-NQ}       & reproduce                                   & 74.21                & 64.208               & \multicolumn{1}{c|}{67.694}  & 82.11                & 84.684               & 80.604               & \multicolumn{1}{c|}{75.594} & 78.008               & 82.042               & 75.348               & \multicolumn{1}{c|}{61.858}     & 91.14                & 81.544               & 73.83                & 72.65                 & 50.94                 & 74.779                   \\ %\cmidrule(l){3-19} 
                               & online                                      & 81.872               & 75.956               & \multicolumn{1}{c|}{76.794}  & 82.658               & 78.068               & 68.194               & \multicolumn{1}{c|}{57.4}   & 61.224               & 60.274               & 50.434               & \multicolumn{1}{c|}{35.06}      & 70.792               & 50.306               & 46.944               & 51.518                & 27.07                 & 60.91025                 \\ \midrule
\multirow{2}{*}{COTTA}         & reproduce                                   & 78.174               & 68.364               & \multicolumn{1}{c|}{64.134}  & 75.464               & 72.054               & 69.796               & \multicolumn{1}{c|}{67.442} & 72.102               & 71.266               & 67.42                & \multicolumn{1}{c|}{62.324}     & 73.612               & 69.648               & 66.752               & 68.402                & 62.074                & 69.31425                 \\ %\cmidrule(l){3-19} 
                               & online                                      & 82.614               & 83.95                & \multicolumn{1}{c|}{83.716}  & 88.692               & 87.1                 & 82.294               & \multicolumn{1}{c|}{75.324} & 75.738               & 76.71                & 66.42                & \multicolumn{1}{c|}{55.338}     & 91.02                & 75.412               & 65.842               & 67.596                & 50.492                & 75.516125                \\ \midrule
\multirow{2}{*}{BN-Adaptation} & reproduce                                   & 84.58                & 83.878               & \multicolumn{1}{c|}{83.788}  & 80.098               & 80.26                & 71.616               & \multicolumn{1}{c|}{60.638} & 65.208               & 65.38                & 51.396               & \multicolumn{1}{c|}{34.388}     & 76.1                 & 54.516               & 49.634               & 59.146                & 24.56                 & 64.074125                \\ %\cmidrule(l){3-19} 
                               & online                                      & 84.58                & 83.878               & \multicolumn{1}{c|}{83.788}  & 80.098               & 80.26                & 71.616               & \multicolumn{1}{c|}{60.638} & 65.208               & 65.38                & 51.396               & \multicolumn{1}{c|}{34.388}     & 76.1                 & 54.516               & 49.634               & 59.146                & 24.56                 & 64.074125                \\ \midrule
\multirow{2}{*}{SHOT}          & reproduce                                   & 75.832               & 68.134               & \multicolumn{1}{c|}{68.088}  & 75.734               & 72.34                & 66.988               & \multicolumn{1}{c|}{58.25}  & 64.776               & 65.378               & 56.498               & \multicolumn{1}{c|}{42.414}     & 73.146               & 53.54                & 49.784               & 54.474                & 34.1                  & 61.21725                 \\ %\cmidrule(l){3-19} 
                               & online                                      & 81.638               & 75.466               & \multicolumn{1}{c|}{73.864}  & 78.158               & 75.288               & 66.248               & \multicolumn{1}{c|}{55.684} & 62.04                & 61.982               & 51.258               & \multicolumn{1}{c|}{37.14}      & 72.72                & 50.53                & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} & 64.77046154              \\ \midrule
\multirow{2}{*}{SHOT-IM}       & reproduce                                   & 76.32                & 68.626               & \multicolumn{1}{c|}{68.5}    & 75.9                 & 72.556               & 67.112               & \multicolumn{1}{c|}{58.198} & 64.806               & 65.358               & 56.37                & \multicolumn{1}{c|}{42.272}     & 73.478               & 53.61                & 49.84                & 54.6                  & 33.85                 & 61.33725                 \\ %\cmidrule(l){3-19} 
                               & online                                      & 80.392               & 72.392               & \multicolumn{1}{c|}{71.246}  & 76.816               & 73.526               & 66.378               & \multicolumn{1}{c|}{56.59}  & 63.17                & 63.39                & 53.642               & \multicolumn{1}{c|}{39.436}     & 72.932               & 51.634               & 48.118               & 53.764                & 31.32                 & 60.921625                \\ \midrule
\multirow{2}{*}{LAME}          & reproduce                                   & 84.962               & 84.108               & \multicolumn{1}{c|}{84.342}  & 84.95                & 84.764               & 73.75                & \multicolumn{1}{c|}{61.274} & 65.79                & 67.07                & 52.15                & \multicolumn{1}{c|}{34.832}     & 83.042               & 56.08                & 51.108               & 60.188                & 24.814                & 65.8265                  \\ %\cmidrule(l){3-19} 
                               & online                                      & 84.928               & 84.05                & \multicolumn{1}{c|}{84.288}  & 84.892               & 84.752               & 73.692               & \multicolumn{1}{c|}{61.246} & 65.742               & 66.968               & 52.084               & \multicolumn{1}{c|}{34.814}     & 82.992               & 56.03                & 51.074               & 60.152                & 24.766                & 65.779375                \\ \midrule
\multirow{2}{*}{PL}            & reproduce                                   & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{}        & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{}       & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{}           & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &                          \\ %\cmidrule(l){3-19} 
                               & online                                      & 84.81                & 82.692               & \multicolumn{1}{c|}{80.416}  & 81.482               & 79.35                & 68.108               & \multicolumn{1}{c|}{56.348} & 62.228               & 62.352               & 49.934               & \multicolumn{1}{c|}{35.162}     & 72.786               & 50.848               & 45.98                & 52.63                 & 26.756                & 61.992625                \\ \midrule
\multirow{2}{*}{SAR}           & reproduce                                   & 69.624               & 62.51                & \multicolumn{1}{c|}{62.636}  & 72.694               & 69.776               & 64.85                & \multicolumn{1}{c|}{57.538} & 63.528               & 63.826               & 52.614               & \multicolumn{1}{c|}{41.104}     & 67.58                & 52.732               & 49.166               & 52.06                 & 34.014                &                          \\ %\cmidrule(l){3-19} 
                               & online                                      & 84.468               & 80.902               & 79.384                       & 81.38                & 78.898               & 68.444               & 56.638                      & 62.502               & 62.596               & 50.882               & 35.784                          & 73.258               & 50.882               & 46.642               & 53.016                & 27.384                & 62.06625                 \\ \bottomrule
                               \bottomrule
                               
\end{tabular}%
}
\end{table*}
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
% \begin{table*}[]
% \resizebox{\textwidth}{!}{%
% \begin{tabular}{cllllllllllllllllll}
% \hline
% \multirow{4}{*}{Method}        & \multicolumn{1}{c}{\multirow{4}{*}{Eval.}}      & \multicolumn{3}{c}{\multirow{2}{*}{Noise}}                                                         & \multicolumn{3}{c}{\multirow{2}{*}{Blur}}                                   & \multicolumn{5}{c}{\multirow{2}{*}{Weather}}                                                                                                                              & \multicolumn{4}{c}{\multirow{2}{*}{Digital}}                                                                                   & \multicolumn{1}{c}{\multirow{4}{*}{val}}    & \multicolumn{1}{c}{\multirow{4}{*}{Average}} \\
%                                & \multicolumn{1}{c}{}                            & \multicolumn{3}{c}{}                                                                               & \multicolumn{3}{c}{}                                                        & \multicolumn{5}{c}{}                                                                                                                                                      & \multicolumn{4}{c}{}                                                                                                           & \multicolumn{1}{c}{}                        & \multicolumn{1}{c}{}                         \\ \cline{3-17}
%                                & \multicolumn{1}{c}{}                            & \multirow{2}{*}{gaussian} & \multirow{2}{*}{shot}  & \multicolumn{1}{l|}{\multirow{2}{*}{impulse}} & \multirow{2}{*}{defocus} & \multirow{2}{*}{glass} & \multirow{2}{*}{motion} & \multicolumn{1}{l|}{\multirow{2}{*}{zoom}}  & \multirow{2}{*}{snow}  & \multirow{2}{*}{frost} & \multirow{2}{*}{fog}   & \multicolumn{1}{l|}{\multirow{2}{*}{brightness}} & \multirow{2}{*}{contrast} & \multirow{2}{*}{elastic} & \multirow{2}{*}{pixelate} & \multicolumn{1}{l|}{\multirow{2}{*}{jpeg}}  & \multicolumn{1}{c}{}                        & \multicolumn{1}{c}{}                         \\
%                                & \multicolumn{1}{c}{}                            &                           &                        & \multicolumn{1}{l|}{}                         &                          &                        &                         & \multicolumn{1}{l|}{}                       &                        &                        &                        & \multicolumn{1}{l|}{}                            &                           &                          &                           & \multicolumn{1}{l|}{}                       & \multicolumn{1}{c}{}                        & \multicolumn{1}{c}{}                         \\ \hline
% \multirow{4}{*}{Tent}          & \multicolumn{1}{l|}{\multirow{2}{*}{reproduce}} & \multirow{2}{*}{71.31}    & \multirow{2}{*}{65.86} & \multicolumn{1}{l|}{\multirow{2}{*}{68.69}}   & \multirow{2}{*}{81.91}   & \multirow{2}{*}{89.20} & \multirow{2}{*}{93.91}  & \multicolumn{1}{l|}{\multirow{2}{*}{96.34}} & \multirow{2}{*}{98.76} & \multirow{2}{*}{99.31} & \multirow{2}{*}{99.29} & \multicolumn{1}{l|}{\multirow{2}{*}{99.23}}      & \multirow{2}{*}{99.61}    & \multirow{2}{*}{99.46}   & \multirow{2}{*}{99.44}    & \multicolumn{1}{l|}{\multirow{2}{*}{99.47}} & \multicolumn{1}{l|}{\multirow{2}{*}{99.35}} & \multirow{2}{*}{91.32}                       \\
%                                & \multicolumn{1}{l|}{}                           &                           &                        & \multicolumn{1}{l|}{}                         &                          &                        &                         & \multicolumn{1}{l|}{}                       &                        &                        &                        & \multicolumn{1}{l|}{}                            &                           &                          &                           & \multicolumn{1}{l|}{}                       & \multicolumn{1}{l|}{}                       &                                              \\ \cline{2-19} 
%                                & \multicolumn{1}{l|}{\multirow{2}{*}{online}}    & \multirow{2}{*}{72.34}    & \multirow{2}{*}{65.77} & \multicolumn{1}{l|}{\multirow{2}{*}{68.54}}   & \multirow{2}{*}{81.52}   & \multirow{2}{*}{88.83} & \multirow{2}{*}{93.73}  & \multicolumn{1}{l|}{\multirow{2}{*}{96.33}} & \multirow{2}{*}{98.80} & \multirow{2}{*}{99.33} & \multirow{2}{*}{99.31} & \multicolumn{1}{l|}{\multirow{2}{*}{99.19}}      & \multirow{2}{*}{99.61}    & \multirow{2}{*}{99.44}   & \multirow{2}{*}{99.42}    & \multicolumn{1}{l|}{\multirow{2}{*}{99.47}} & \multicolumn{1}{l|}{\multirow{2}{*}{99.36}} & \multirow{2}{*}{91.31}                       \\
%                                & \multicolumn{1}{l|}{}                           &                           &                        & \multicolumn{1}{l|}{}                         &                          &                        &                         & \multicolumn{1}{l|}{}                       &                        &                        &                        & \multicolumn{1}{l|}{}                            &                           &                          &                           & \multicolumn{1}{l|}{}                       & \multicolumn{1}{l|}{}                       &                                              \\ \hline
% \multirow{4}{*}{AdaBN}         & \multicolumn{1}{l|}{\multirow{2}{*}{reproduce}} & \multirow{2}{*}{84.91}    & \multirow{2}{*}{84.05} & \multicolumn{1}{l|}{\multirow{2}{*}{84.27}}   & \multirow{2}{*}{84.88}   & \multirow{2}{*}{84.74} & \multirow{2}{*}{73.66}  & \multicolumn{1}{l|}{\multirow{2}{*}{61.25}} & \multirow{2}{*}{65.71} & \multirow{2}{*}{66.97} & \multirow{2}{*}{52.03} & \multicolumn{1}{l|}{\multirow{2}{*}{34.78}}      & \multirow{2}{*}{83.00}    & \multirow{2}{*}{56.01}   & \multirow{2}{*}{51.03}    & \multicolumn{1}{l|}{\multirow{2}{*}{60.15}} & \multicolumn{1}{l|}{\multirow{2}{*}{24.77}} & \multirow{2}{*}{65.76}                       \\
%                                & \multicolumn{1}{l|}{}                           &                           &                        & \multicolumn{1}{l|}{}                         &                          &                        &                         & \multicolumn{1}{l|}{}                       &                        &                        &                        & \multicolumn{1}{l|}{}                            &                           &                          &                           & \multicolumn{1}{l|}{}                       & \multicolumn{1}{l|}{}                       &                                              \\ \cline{2-19} 
%                                & \multicolumn{1}{l|}{\multirow{2}{*}{online}}    & \multirow{2}{*}{84.91}    & \multirow{2}{*}{84.05} & \multicolumn{1}{l|}{\multirow{2}{*}{84.27}}   & \multirow{2}{*}{84.88}   & \multirow{2}{*}{84.74} & \multirow{2}{*}{73.66}  & \multicolumn{1}{l|}{\multirow{2}{*}{61.25}} & \multirow{2}{*}{65.71} & \multirow{2}{*}{66.97} & \multirow{2}{*}{52.03} & \multicolumn{1}{l|}{\multirow{2}{*}{34.78}}      & \multirow{2}{*}{83.00}    & \multirow{2}{*}{56.01}   & \multirow{2}{*}{51.03}    & \multicolumn{1}{l|}{\multirow{2}{*}{60.15}} & \multicolumn{1}{l|}{\multirow{2}{*}{24.77}} & \multirow{2}{*}{65.76}                       \\
%                                & \multicolumn{1}{l|}{}                           &                           &                        & \multicolumn{1}{l|}{}                         &                          &                        &                         & \multicolumn{1}{l|}{}                       &                        &                        &                        & \multicolumn{1}{l|}{}                            &                           &                          &                           & \multicolumn{1}{l|}{}                       & \multicolumn{1}{l|}{}                       &                                              \\ \hline
% \multirow{4}{*}{ETA}           & \multicolumn{1}{l|}{\multirow{2}{*}{reproduce}} & \multirow{2}{*}{65.22}    & \multirow{2}{*}{59.26} & \multicolumn{1}{l|}{\multirow{2}{*}{60.50}}   & \multirow{2}{*}{70.09}   & \multirow{2}{*}{68.33} & \multirow{2}{*}{62.98}  & \multicolumn{1}{l|}{\multirow{2}{*}{56.34}} & \multirow{2}{*}{58.85} & \multirow{2}{*}{61.07} & \multirow{2}{*}{48.40} & \multicolumn{1}{l|}{\multirow{2}{*}{39.25}}      & \multirow{2}{*}{58.13}    & \multirow{2}{*}{48.90}   & \multirow{2}{*}{44.88}    & \multicolumn{1}{l|}{\multirow{2}{*}{48.64}} & \multicolumn{1}{l|}{\multirow{2}{*}{32.90}} & \multirow{2}{*}{55.23}                       \\
%                                & \multicolumn{1}{l|}{}                           &                           &                        & \multicolumn{1}{l|}{}                         &                          &                        &                         & \multicolumn{1}{l|}{}                       &                        &                        &                        & \multicolumn{1}{l|}{}                            &                           &                          &                           & \multicolumn{1}{l|}{}                       & \multicolumn{1}{l|}{}                       &                                              \\ \cline{2-19} 
%                                & \multicolumn{1}{l|}{\multirow{2}{*}{online}}    & \multirow{2}{*}{77.11}    & \multirow{2}{*}{67.52} & \multicolumn{1}{l|}{\multirow{2}{*}{65.94}}   & \multirow{2}{*}{75.39}   & \multirow{2}{*}{70.68} & \multirow{2}{*}{64.76}  & \multicolumn{1}{l|}{\multirow{2}{*}{57.63}} & \multirow{2}{*}{63.20} & \multirow{2}{*}{62.56} & \multirow{2}{*}{52.90} & \multicolumn{1}{l|}{\multirow{2}{*}{40.16}}      & \multirow{2}{*}{64.18}    & \multirow{2}{*}{50.60}   & \multirow{2}{*}{46.58}    & \multicolumn{1}{l|}{\multirow{2}{*}{50.12}} & \multicolumn{1}{l|}{\multirow{2}{*}{32.48}} & \multirow{2}{*}{58.86}                       \\
%                                & \multicolumn{1}{l|}{}                           &                           &                        & \multicolumn{1}{l|}{}                         &                          &                        &                         & \multicolumn{1}{l|}{}                       &                        &                        &                        & \multicolumn{1}{l|}{}                            &                           &                          &                           & \multicolumn{1}{l|}{}                       & \multicolumn{1}{l|}{}                       &                                              \\ \hline
% \multirow{4}{*}{EATA}          & \multicolumn{1}{l|}{\multirow{2}{*}{reproduce}} & \multirow{2}{*}{65.22}    & \multirow{2}{*}{59.26} & \multicolumn{1}{l|}{\multirow{2}{*}{60.50}}   & \multirow{2}{*}{70.09}   & \multirow{2}{*}{68.33} & \multirow{2}{*}{62.98}  & \multicolumn{1}{l|}{\multirow{2}{*}{56.34}} & \multirow{2}{*}{58.85} & \multirow{2}{*}{61.07} & \multirow{2}{*}{48.40} & \multicolumn{1}{l|}{\multirow{2}{*}{39.25}}      & \multirow{2}{*}{58.13}    & \multirow{2}{*}{48.90}   & \multirow{2}{*}{44.88}    & \multicolumn{1}{l|}{\multirow{2}{*}{48.64}} & \multicolumn{1}{l|}{\multirow{2}{*}{32.90}} & \multirow{2}{*}{55.23}                       \\
%                                & \multicolumn{1}{l|}{}                           &                           &                        & \multicolumn{1}{l|}{}                         &                          &                        &                         & \multicolumn{1}{l|}{}                       &                        &                        &                        & \multicolumn{1}{l|}{}                            &                           &                          &                           & \multicolumn{1}{l|}{}                       & \multicolumn{1}{l|}{}                       &                                              \\ \cline{2-19} 
%                                & \multicolumn{1}{l|}{\multirow{2}{*}{online}}    & \multirow{2}{*}{77.11}    & \multirow{2}{*}{67.52} & \multicolumn{1}{l|}{\multirow{2}{*}{65.94}}   & \multirow{2}{*}{75.39}   & \multirow{2}{*}{70.68} & \multirow{2}{*}{64.76}  & \multicolumn{1}{l|}{\multirow{2}{*}{57.63}} & \multirow{2}{*}{63.20} & \multirow{2}{*}{62.56} & \multirow{2}{*}{52.90} & \multicolumn{1}{l|}{\multirow{2}{*}{40.16}}      & \multirow{2}{*}{64.18}    & \multirow{2}{*}{50.60}   & \multirow{2}{*}{46.58}    & \multicolumn{1}{l|}{\multirow{2}{*}{50.12}} & \multicolumn{1}{l|}{\multirow{2}{*}{32.48}} & \multirow{2}{*}{58.86}                       \\
%                                & \multicolumn{1}{l|}{}                           &                           &                        & \multicolumn{1}{l|}{}                         &                          &                        &                         & \multicolumn{1}{l|}{}                       &                        &                        &                        & \multicolumn{1}{l|}{}                            &                           &                          &                           & \multicolumn{1}{l|}{}                       & \multicolumn{1}{l|}{}                       &                                              \\ \hline
% \multirow{4}{*}{TTAC-NQ}       & \multicolumn{1}{l|}{\multirow{2}{*}{reproduce}} & \multirow{2}{*}{74.21}    & \multirow{2}{*}{64.21} & \multicolumn{1}{l|}{\multirow{2}{*}{67.69}}   & \multirow{2}{*}{82.11}   & \multirow{2}{*}{84.68} & \multirow{2}{*}{80.60}  & \multicolumn{1}{l|}{\multirow{2}{*}{75.59}} & \multirow{2}{*}{78.01} & \multirow{2}{*}{82.04} & \multirow{2}{*}{75.35} & \multicolumn{1}{l|}{\multirow{2}{*}{61.86}}      & \multirow{2}{*}{91.14}    & \multirow{2}{*}{81.54}   & \multirow{2}{*}{73.83}    & \multicolumn{1}{l|}{\multirow{2}{*}{72.65}} & \multicolumn{1}{l|}{\multirow{2}{*}{50.94}} & \multirow{2}{*}{74.78}                       \\
%                                & \multicolumn{1}{l|}{}                           &                           &                        & \multicolumn{1}{l|}{}                         &                          &                        &                         & \multicolumn{1}{l|}{}                       &                        &                        &                        & \multicolumn{1}{l|}{}                            &                           &                          &                           & \multicolumn{1}{l|}{}                       & \multicolumn{1}{l|}{}                       &                                              \\ \cline{2-19} 
%                                & \multicolumn{1}{l|}{\multirow{2}{*}{online}}    & \multirow{2}{*}{81.87}    & \multirow{2}{*}{75.96} & \multicolumn{1}{l|}{\multirow{2}{*}{76.79}}   & \multirow{2}{*}{82.66}   & \multirow{2}{*}{78.07} & \multirow{2}{*}{68.19}  & \multicolumn{1}{l|}{\multirow{2}{*}{57.40}} & \multirow{2}{*}{61.22} & \multirow{2}{*}{60.27} & \multirow{2}{*}{50.43} & \multicolumn{1}{l|}{\multirow{2}{*}{35.06}}      & \multirow{2}{*}{70.79}    & \multirow{2}{*}{50.31}   & \multirow{2}{*}{46.94}    & \multicolumn{1}{l|}{\multirow{2}{*}{51.52}} & \multicolumn{1}{l|}{\multirow{2}{*}{27.07}} & \multirow{2}{*}{60.91}                       \\
%                                & \multicolumn{1}{l|}{}                           &                           &                        & \multicolumn{1}{l|}{}                         &                          &                        &                         & \multicolumn{1}{l|}{}                       &                        &                        &                        & \multicolumn{1}{l|}{}                            &                           &                          &                           & \multicolumn{1}{l|}{}                       & \multicolumn{1}{l|}{}                       &                                              \\ \hline
% \multirow{4}{*}{COTTA}         & \multicolumn{1}{l|}{\multirow{2}{*}{reproduce}} & \multirow{2}{*}{78.17}    & \multirow{2}{*}{68.36} & \multicolumn{1}{l|}{\multirow{2}{*}{64.13}}   & \multirow{2}{*}{75.46}   & \multirow{2}{*}{72.05} & \multirow{2}{*}{69.80}  & \multicolumn{1}{l|}{\multirow{2}{*}{67.44}} & \multirow{2}{*}{72.10} & \multirow{2}{*}{71.27} & \multirow{2}{*}{67.42} & \multicolumn{1}{l|}{\multirow{2}{*}{62.32}}      & \multirow{2}{*}{73.61}    & \multirow{2}{*}{69.65}   & \multirow{2}{*}{66.75}    & \multicolumn{1}{l|}{\multirow{2}{*}{68.40}} & \multicolumn{1}{l|}{\multirow{2}{*}{62.07}} & \multirow{2}{*}{69.31}                       \\
%                                & \multicolumn{1}{l|}{}                           &                           &                        & \multicolumn{1}{l|}{}                         &                          &                        &                         & \multicolumn{1}{l|}{}                       &                        &                        &                        & \multicolumn{1}{l|}{}                            &                           &                          &                           & \multicolumn{1}{l|}{}                       & \multicolumn{1}{l|}{}                       &                                              \\ \cline{3-19} 
%                                & \multirow{2}{*}{online}                         & \multirow{2}{*}{82.61}    & \multirow{2}{*}{83.95} & \multirow{2}{*}{83.72}                        & \multirow{2}{*}{88.69}   & \multirow{2}{*}{87.10} & \multirow{2}{*}{82.29}  & \multirow{2}{*}{75.32}                      & \multirow{2}{*}{75.74} & \multirow{2}{*}{76.71} & \multirow{2}{*}{66.42} & \multirow{2}{*}{55.34}                           & \multirow{2}{*}{91.02}    & \multirow{2}{*}{75.41}   & \multirow{2}{*}{65.84}    & \multirow{2}{*}{67.60}                      & \multirow{2}{*}{50.49}                      & \multirow{2}{*}{75.52}                       \\
%                                &                                                 &                           &                        &                                               &                          &                        &                         &                                             &                        &                        &                        &                                                  &                           &                          &                           &                                             &                                             &                                              \\ \cline{1-1}
% \multirow{4}{*}{BN-Adaptation} & \multirow{2}{*}{reproduce}                      & \multirow{2}{*}{84.58}    & \multirow{2}{*}{83.88} & \multirow{2}{*}{83.79}                        & \multirow{2}{*}{80.10}   & \multirow{2}{*}{80.26} & \multirow{2}{*}{71.62}  & \multirow{2}{*}{60.64}                      & \multirow{2}{*}{65.21} & \multirow{2}{*}{65.38} & \multirow{2}{*}{51.40} & \multirow{2}{*}{34.39}                           & \multirow{2}{*}{76.10}    & \multirow{2}{*}{54.52}   & \multirow{2}{*}{49.63}    & \multirow{2}{*}{59.15}                      & \multirow{2}{*}{24.56}                      & \multirow{2}{*}{64.07}                       \\
%                                &                                                 &                           &                        &                                               &                          &                        &                         &                                             &                        &                        &                        &                                                  &                           &                          &                           &                                             &                                             &                                              \\
%                                & \multirow{2}{*}{online}                         & \multirow{2}{*}{84.58}    & \multirow{2}{*}{83.88} & \multirow{2}{*}{83.79}                        & \multirow{2}{*}{80.10}   & \multirow{2}{*}{80.26} & \multirow{2}{*}{71.62}  & \multirow{2}{*}{60.64}                      & \multirow{2}{*}{65.21} & \multirow{2}{*}{65.38} & \multirow{2}{*}{51.40} & \multirow{2}{*}{34.39}                           & \multirow{2}{*}{76.10}    & \multirow{2}{*}{54.52}   & \multirow{2}{*}{49.63}    & \multirow{2}{*}{59.15}                      & \multirow{2}{*}{24.56}                      & \multirow{2}{*}{64.07}                       \\
%                                &                                                 &                           &                        &                                               &                          &                        &                         &                                             &                        &                        &                        &                                                  &                           &                          &                           &                                             &                                             &                                              \\
% \multirow{4}{*}{SHOT}          & \multirow{2}{*}{reproduce}                      & \multirow{2}{*}{75.83}    & \multirow{2}{*}{68.13} & \multirow{2}{*}{68.09}                        & \multirow{2}{*}{75.73}   & \multirow{2}{*}{72.34} & \multirow{2}{*}{66.99}  & \multirow{2}{*}{58.25}                      & \multirow{2}{*}{64.78} & \multirow{2}{*}{65.38} & \multirow{2}{*}{56.50} & \multirow{2}{*}{42.41}                           & \multirow{2}{*}{73.15}    & \multirow{2}{*}{53.54}   & \multirow{2}{*}{49.78}    & \multirow{2}{*}{54.47}                      & \multirow{2}{*}{34.10}                      & \multirow{2}{*}{61.22}                       \\
%                                &                                                 &                           &                        &                                               &                          &                        &                         &                                             &                        &                        &                        &                                                  &                           &                          &                           &                                             &                                             &                                              \\
%                                & \multirow{2}{*}{online}                         & \multirow{2}{*}{81.64}    & \multirow{2}{*}{75.47} & \multirow{2}{*}{73.86}                        & \multirow{2}{*}{78.16}   & \multirow{2}{*}{75.29} & \multirow{2}{*}{66.25}  & \multirow{2}{*}{55.68}                      & \multirow{2}{*}{62.04} & \multirow{2}{*}{61.98} & \multirow{2}{*}{51.26} & \multirow{2}{*}{37.14}                           & \multirow{2}{*}{72.72}    & \multirow{2}{*}{50.53}   & \multirow{2}{*}{}         & \multirow{2}{*}{}                           & \multirow{2}{*}{}                           & \multirow{2}{*}{64.77}                       \\
%                                &                                                 &                           &                        &                                               &                          &                        &                         &                                             &                        &                        &                        &                                                  &                           &                          &                           &                                             &                                             &                                              \\
% \multirow{4}{*}{SHOT-IM}       & \multirow{2}{*}{reproduce}                      & \multirow{2}{*}{76.32}    & \multirow{2}{*}{68.63} & \multirow{2}{*}{68.50}                        & \multirow{2}{*}{75.90}   & \multirow{2}{*}{72.56} & \multirow{2}{*}{67.11}  & \multirow{2}{*}{58.20}                      & \multirow{2}{*}{64.81} & \multirow{2}{*}{65.36} & \multirow{2}{*}{56.37} & \multirow{2}{*}{42.27}                           & \multirow{2}{*}{73.48}    & \multirow{2}{*}{53.61}   & \multirow{2}{*}{49.84}    & \multirow{2}{*}{54.60}                      & \multirow{2}{*}{33.85}                      & \multirow{2}{*}{61.34}                       \\
%                                &                                                 &                           &                        &                                               &                          &                        &                         &                                             &                        &                        &                        &                                                  &                           &                          &                           &                                             &                                             &                                              \\
%                                & \multirow{2}{*}{online}                         & \multirow{2}{*}{80.39}    & \multirow{2}{*}{72.39} & \multirow{2}{*}{71.25}                        & \multirow{2}{*}{76.82}   & \multirow{2}{*}{73.53} & \multirow{2}{*}{66.38}  & \multirow{2}{*}{56.59}                      & \multirow{2}{*}{63.17} & \multirow{2}{*}{63.39} & \multirow{2}{*}{53.64} & \multirow{2}{*}{39.44}                           & \multirow{2}{*}{72.93}    & \multirow{2}{*}{51.63}   & \multirow{2}{*}{48.12}    & \multirow{2}{*}{53.76}                      & \multirow{2}{*}{31.32}                      & \multirow{2}{*}{60.92}                       \\
% \multirow{4}{*}{LAME}          & \multirow{2}{*}{reproduce}                      & \multirow{2}{*}{84.96}    & \multirow{2}{*}{84.11} & \multirow{2}{*}{84.34}                        & \multirow{2}{*}{84.95}   & \multirow{2}{*}{84.76} & \multirow{2}{*}{73.75}  & \multirow{2}{*}{61.27}                      & \multirow{2}{*}{65.79} & \multirow{2}{*}{67.07} & \multirow{2}{*}{52.15} & \multirow{2}{*}{34.83}                           & \multirow{2}{*}{83.04}    & \multirow{2}{*}{56.08}   & \multirow{2}{*}{51.11}    & \multirow{2}{*}{60.19}                      & \multirow{2}{*}{24.81}                      & \multirow{2}{*}{65.83}                          \\
%                                & \multirow{2}{*}{online}                         & \multirow{2}{*}{84.93}    & \multirow{2}{*}{84.05} & \multirow{2}{*}{84.29}                        & \multirow{2}{*}{84.89}   & \multirow{2}{*}{84.75} & \multirow{2}{*}{73.69}  & \multirow{2}{*}{61.25}                      & \multirow{2}{*}{65.74} & \multirow{2}{*}{66.97} & \multirow{2}{*}{52.08} & \multirow{2}{*}{34.81}                           & \multirow{2}{*}{82.99}    & \multirow{2}{*}{56.03}   & \multirow{2}{*}{51.07}    & \multirow{2}{*}{60.15}                      & \multirow{2}{*}{24.77}                      & \multirow{2}{*}{65.78}                       \\
% \multirow{4}{*}{PL}            & \multirow{2}{*}{reproduce}                      & \multirow{2}{*}{}         & \multirow{2}{*}{}      & \multirow{2}{*}{}                             & \multirow{2}{*}{}        & \multirow{2}{*}{}      & \multirow{2}{*}{}       & \multirow{2}{*}{}                           & \multirow{2}{*}{}      & \multirow{2}{*}{}      & \multirow{2}{*}{}      & \multirow{2}{*}{}                                & \multirow{2}{*}{}         & \multirow{2}{*}{}        & \multirow{2}{*}{}         & \multirow{2}{*}{}                           & \multirow{2}{*}{}                           & \multirow{2}{*}{}                            \\
%                                & \multirow{2}{*}{online}                         & \multirow{2}{*}{84.81}    & \multirow{2}{*}{82.69} & \multirow{2}{*}{80.42}                        & \multirow{2}{*}{81.48}   & \multirow{2}{*}{79.35} & \multirow{2}{*}{68.11}  & \multirow{2}{*}{56.35}                      & \multirow{2}{*}{62.23} & \multirow{2}{*}{62.35} & \multirow{2}{*}{49.93} & \multirow{2}{*}{35.16}                           & \multirow{2}{*}{72.79}    & \multirow{2}{*}{50.85}   & \multirow{2}{*}{45.98}    & \multirow{2}{*}{52.63}                      & \multirow{2}{*}{26.76}                      & \multirow{2}{*}{61.99}                       \\
% \multirow{4}{*}{SAR}           & \multirow{2}{*}{reproduce}                      & \multirow{2}{*}{69.62}    & \multirow{2}{*}{62.51} & \multirow{2}{*}{62.64}                        & \multirow{2}{*}{72.69}   & \multirow{2}{*}{69.78} & \multirow{2}{*}{64.85}  & \multirow{2}{*}{57.54}                      & \multirow{2}{*}{63.53} & \multirow{2}{*}{63.83} & \multirow{2}{*}{52.61} & \multirow{2}{*}{41.10}                           & \multirow{2}{*}{67.58}    & \multirow{2}{*}{52.73}   & \multirow{2}{*}{49.17}    & \multirow{2}{*}{52.06}                      & \multirow{2}{*}{34.01}                      & \multirow{2}{*}{}          \\
%                                & \multirow{2}{*}{online}                         & \multirow{2}{*}{84.47}    & \multirow{2}{*}{80.90} & \multirow{2}{*}{79.38}                        & \multirow{2}{*}{81.38}   & \multirow{2}{*}{78.90} & \multirow{2}{*}{68.44}  & \multirow{2}{*}{56.64}                      & \multirow{2}{*}{62.50} & \multirow{2}{*}{62.60} & \multirow{2}{*}{50.88} & \multirow{2}{*}{35.78}                           & \multirow{2}{*}{73.26}    & \multirow{2}{*}{50.88}   & \multirow{2}{*}{46.64}    & \multirow{2}{*}{53.02}                      & \multirow{2}{*}{27.38}                      & \multirow{2}{*}{62.07}                                           
% \end{tabular}%
% }
% \end{table*}

==> Tables/lifelong_graphs_3dcc.tex <==

\begin{table*}[ccc]

\includegraphics[width=.3\linewidth]{Figures/Lifelong/ETA_3dcc.pdf}&& \includegraphics[width=.3\linewidth]{Figures/Lifelong/SAR_3dcc.pdf}\\

\includegraphics[width=.3\linewidth]{Figures/Lifelong/EATA_3dcc.pdf}&
\includegraphics[width=.3\linewidth]{Figures/Lifelong/TTAC-NQ.pdf} & \includegraphics[width=.3\linewidth]{Figures/Lifelong/COTTA_3dcc.pdf} \\ 

\includegraphics[width=.3\linewidth]{Figures/Lifelong/Tent_3dcc.pdf}& \includegraphics[width=.3\linewidth]{Figures/Lifelong/SHOT_3dcc.pdf}&
\includegraphics[width=.3\linewidth]{Figures/Lifelong/SHOT-IM.pdf} \\ 
Imagenet 3dcc lifelong 

\end{table*}
